Plane-filling curves on all uniform grids

We describe a search for plane-filling curves traversing all edges of a grid once. The curves are given by Lindenmayer systems with only one non-constant letter. All such curves for small orders on three grids have been found. For all uniform grids we show how curves traversing all points once can be obtained from the curves found. Curves traversing all edges once are described for the four uniform grids where they exist.

==> makefile <==

TNT=test "$$?" -eq "1" ## tricky: The Not-Trick

LATEX=latex -interaction=nonstopmode
#PDFLATEX=pdflatex -interaction=nonstopmode
PDFLATEX=pdflatex -interaction=nonstopmode --synctex=1

BASE=arndt-curve-search

ALLSRC=$(BASE)*.tex bib.tex

.PHONY: default
default: all

.PHONY: dvi
dvi:
	rm -rf $(BASE).aux
	$(LATEX) -src-specials $(BASE).tex
	$(LATEX) -src-specials $(BASE).tex

.PHONY: pdf
pdf:
	rm -rf $(BASE).aux
	$(PDFLATEX) $(BASE).tex
	$(PDFLATEX) $(BASE).tex
	$(PDFLATEX) $(BASE).tex

.PHONY: all
all: chk dvi pdf
#	dvips $(BASE).dvi
#	pdf2ps $(BASE).pdf
	: '[$@] done'

.PHONY: check chk
check chk:
	./chk-bib-sort.pl < bib.tex
	zsh ./check-figures.zsh

.PHONY: ichkstutter ## check for stutter (like "is is")
ichkstutter:
	: '[$@]'
	for f in $(ALLSRC) ; do dupwords.pl $$f; done
#	/bin/zsh scripts/chk-double-words.zsh

SCRIPTDIR=./scripts/
.PHONY: ichkspell  ##  spell-check-oids
ichkspell:
	: '[$@]'
	$(SCRIPTDIR)/chkspell.zsh


.PHONY: Etarget
Etarget: all

.PHONY: Etarget2
Etarget2: all


.PHONY: vv
vv:
#	xdvi $(BASE).dvi &
	mupdf -r 130 $(BASE).pdf &

.PHONY: ed-tex
ed-tex:
	emacs bib.tex arndt-curve-search*.tex &



.PHONY: ctfigures
ctfigures:
	: 'In all sources:'
	grep -F '\begin{figure}' $(ALLSRC) | grep -vF ':%' | wc -l
	grep  '^[^%].*includegraphics' $(ALLSRC) | grep -vF ':%' | wc -l
	: 'Actually used:'
#	grep -F 'Package pdftex.def Info:' $(BASE).log | wc -l
	grep -F 'Requested size: ' $(BASE).log | wc -l

.PHONY: snapshot
snapshot:
#	cp -iv $(BASE).tex  attic/$(BASE)-$$(date +'%Y.%m.%d-%Hh%M').tex
	D=$(BASE)-$$(date +'%Y.%m.%d-%Hh%M'); mkdir attic/$$D; cp -auvi $(ALLSRC) attic/$$D


.PHONY: clean
clean:
	rm -rf $(BASE).aux
	rm -rf $(BASE).toc
	rm -rf $(BASE).log
	rm -rf $(BASE).out
	rm -rf $(BASE).brf
	rm -rf $(BASE).synctex
	rm -rf $(BASE).synctex.gz


TMPD=/dev/shm/
DDD=arndt-curve-search/
.PHONY: arxiv
arxiv:
	-rm -rf $(TMPD)/$(DDD)
	mkdir $(TMPD)/$(DDD)
	cp -auvi arndt-curve-search*tex $(TMPD)/$(DDD)
	cp -auvi bib.tex $(TMPD)/$(DDD)
	cp -rauvi figures/ $(TMPD)/$(DDD)
	(cd $(TMPD)/$(DDD) && pdflatex arndt-curve-search.tex; )
	(cd $(TMPD)/$(DDD) && pdflatex arndt-curve-search.tex; )
	(cd $(TMPD)/$(DDD) &&  mupdf arndt-curve-search.pdf; )
	(cd $(TMPD)/ && tar cvzf $(TMPD)/curve-search.tar.gz $(DDD); )
	ls -lF $(TMPD)/curve-search.tar.gz


### end of file

